Test-Time Adaptation via Conjugate Pseudo-labels

Test-time adaptation (TTA) refers to adapting neural networks to distribution shifts, with access to only the unlabeled test samples from the new domain at test-time. Prior TTA methods optimize over unsupervised objectives such as the entropy of model predictions in TENT [Wang et al., 2021], but it is unclear what exactly makes a good TTA loss. In this paper, we start by presenting a surprising phenomenon: if we attempt to meta-learn the best possible TTA loss over a wide class of functions, then we recover a function that is remarkably similar to (a temperature-scaled version of) the softmax-entropy employed by TENT. This only holds, however, if the classifier we are adapting is trained via cross-entropy; if trained via squared loss, a different best TTA loss emerges. To explain this phenomenon, we analyze TTA through the lens of the training losses's convex conjugate. We show that under natural conditions, this (unsupervised) conjugate function can be viewed as a good local approximation to the original supervised loss and indeed, it recovers the best losses found by meta-learning. This leads to a generic recipe that can be used to find a good TTA loss for any given supervised training loss function of a general class. Empirically, our approach consistently dominates other baselines over a wide range of benchmarks. Our approach is particularly of interest when applied to classifiers trained with novel loss functions, e.g., the recently-proposed PolyLoss, where it differs substantially from (and outperforms) an entropy-based loss. Further, we show that our approach can also be interpreted as a kind of self-training using a very specific soft label, which we refer to as the conjugate pseudolabel. Overall, our method provides a broad framework for better understanding and improving test-time adaptation. Code is available at https://github.com/locuslab/tta_conjugate.

==> method.tex <==
\section{Method : Conjugate Pseudo Labeling}\label{sec:method}
In this section, we propose a new test time adaptation loss function, motivated by our observations from the previous section where we attempted to learn an optimal adaptation loss via meta-learning. First, we show that the framework of conjugate functions precisely captures our empirical meta learning observations (Section~\ref{sec:conjugate}). Next, we propose a general algorithm for test-time adaptation of classifiers based on the conjugate formulation (Section~\ref{sec:conjugate-algo}). Finally, we provide some interesting interpretations of our algorithm and connect it to the standard adaptation objectives in the literature. 

% The meta loss learning experiments from the previous section lead us towards taking into consideration the supervised learning objective used for training the source model while designing the test time adaptation loss/objective. In this section, we formalize the relation between the learnt TTA objective and supervised train loss of the source classifier, based on our observations from the previous section. 

\subsection{The conjugate adaptation loss}
\label{sec:conjugate}
Recall from Section~\ref{sec:meta-loss} that our search for the ``optimal'' test-time adaptation loss via meta-learning revealed that (i) the ``optimal'' loss function depends on the training loss of the base classifier, and was independent of network architecture, training epochs and regularization (ii) for cross-entropy, the ``optimal'' loss was (temperature scaled) entropy of network predictions and for the squared loss, the ``optimal'' loss was the squared loss on network predictions. The simple form of the learnt adaptation loss in each case suggests a deeper connection between the training loss and the learnt adaptation loss. In this section, we show that the learnt adaptation loss appears to take the form of the \emph{conjugate} of the training loss function. 
\begin{definition}[conjugate function]
\label{def:conjugate}For a function $f:\R^K \mapsto \R$, we define the conjugate function $\conjf{f}(y)$ as follows. 
\begin{align}
    \conjf{f}(y) &= \sup\limits_{z \in \R^k} \big(z^\top y - f(z)\big).
\end{align}
\end{definition}
The conjugate function has several interesting properties which make it an important concept in convex analysis. In this work, the following property is of particular relevance.
\begin{remark} If $f:\R^K \mapsto \R$ is convex and differentiable, the supremum in Definition~\ref{def:conjugate} satisfies $y = \nabla f(z)$, and hence, $\conjf{f}(\nabla f(z)) = z^\top \nabla f(z) - f(z)$.
\end{remark}
Finally, we define an adaptation loss based on the conjugate function.

\begin{definition}[conjugate adaptation loss]
\label{def:conjugateadapt}Consider a loss function $\ell:\R^K \times \mathcal{Y}$ that takes the form $\ell(z, y) = f(z) - y^\top z$. We define the conjugate adaptation loss $\conjloss{\ell}(z): \R^K \mapsto \R$ as follows. 
\begin{align}
\label{eqn:conjugateadapt}
    \conjloss{\ell}(z) = -\conjf{f}(\nabla f(z)) = f(z) -  z^\top \nabla f(z).
\end{align}
\end{definition}

\paragraph{Connection to meta-loss observations.}
We compute the conjugate adaptation losses for the training loss we experimented with in Section~\ref{sec:meta-loss}.
\begin{enumerate}
    \item Consider the popular cross-entropy loss $\ellxent(z, y)$ which can be written as $\ellxent(z, y) = \logsumexp(z) - z^\top y$, where $\logsumexp(z) = \log \sum \limits_{k=1}^K \exp(z_k)$. From Equation~\ref{eqn:conjugateadapt}, the corresponding conjugate adaptation loss $\conjloss{\ell}_\text{xent}(z) = \sum\limits_{k=1}^K \softmax(z)_k \log \Big( \softmax(z)_k$ \Big), which matches the learnt meta loss upto a temperature scaling factor. 
\item 
Similarly, for the square loss $\ellsq(z, y) = (z-y)^2 = (1/2)z^2 - y^\top z$, the corresponding conjugate adaptation loss $\conjloss{\ell}_\text{sq}(z) = (-1/2) z^2$ which again matches the learnt meta-loss when using a classifier trained with the squared loss.  
\end{enumerate}
These observations suggest that we should use the conjugate adaptation loss of the loss function used to train the source classifier during test-time adaptation. In the next section, we explore this idea formally. We also draw intriguing connections to the classic self-training and pseudolabeling framework, and discuss some intuition for why such an adaptation loss might make sense. 

\subsection{Conjugate functions and pseudo-labeling}
\label{sec:cpl}
Recall that our empirical experiments suggested that we should minimize the conjugate adaptation loss (Definition~\ref{def:conjugateadapt}) during test-time adaptation. 

Formally, suppose we have a classifier $\theta$ that makes predictions $h_\theta(x): \sX \mapsto \R^K$. The conjugate adaptation loss~\refeqn{conjugateadapt} can be written as follows. 
% Let $\theta_0$ be the ``source'' classifier obtained be minimizing the empirical risk $\lsource(\theta) = \sum\limits_{(x, y) \in \dsource} \ell( h_\theta(x), y)$, for some loss function $\ell(z, y) = f(z) - y^\top z$. Given a batch of unlabeled samples $x$ at test-time, we propose to take a gradient step to minimize the conjugate adaptation loss, i.e.,  
\begin{align}
    \conjloss{\ell}(h_\theta(x)) &= f(h_\theta(x)) - h_\theta(x)^\top \nabla f(h_\theta(x)) \\
    \label{eqn:cpl}
    &= \ell\Big(\underbrace{h_\theta(x)}_{\text{predictions}}, \underbrace{\nabla f(h_\theta(x))}_{\text{pseudo-labels}} \Big). 
\end{align}
\ar{Should probably have self-training in preliminaries}
We find that taking gradient steps in the direction of the conjugate adaptation loss corresponds to self-training with \emph{instantaneous conjugate pseudo-labels} given by $\nabla f(h_\theta(x))$.
Self-training is one of the oldest frameworks in semisupervised learning, and we find that our proposed conjugate adaptation loss, though superficially very different, is essentially self-training with two important caveats. 

First, we use a specific form of pseudo-labels $\nabla f(h_\theta(z))$ that came out of the conjugate formalism of Section~\ref{sec:conjugate}. For the cross-entropy loss, the pseudo-labels correspond to the standard softmax normalization of the predictions. However, for other loss functions, the ``right'' pseudo-labels take a different form. 

Second, we use instantaneous pseudo-labels, i.e. the pseudo-labels are constantly updated rather than being computed just once from the source classifier (as is the standard in self-training). Some prior works like \citet{learning_selftrain}, \citet{momentum_pl} have documented the improvement in performance when using instantaneous pseudo-labels over precomputed pseudo-labels, and they lend further support to the benefits of our proposed conjugate pseudo-labeling approach. 

Several heuristic variants of self-training and other adaptation losses have been proposed like \citet{rpl}, \citet{memo} and \citet{contrastive_tta}. We find that with the right pseudo-labeling (as provided by the conjugate in~\refeqn{cpl}) and by tuning a temperature parameter that governs the scaling of the predictions, we outperform or match other proposed adaptation approaches empirically on a variety of benchmarks (Section~\ref{sec:experiments}). 

Thus the conjugate formalism reveals an intriguing connection between a possible ``optimal'' adaptation loss and the classic framework of self-training, while providing a clean general approach that improves over previous adaptation approaches. 

\subsection{Test-time adaptation via conjugate pseudo-labeling}
\label{sec:conjugatealgo}
In this section, we put all the pieces together to propose our new approach of test-time adaptation via \emph{conjugate pseudo-labeling}. The key idea is to take a step in the direction of the negative gradient of the conjugate adaptation loss evaluated on each batch at test-time. We call our approach conjugate pseudo-labeling due to its connections to the classic algorithm of self-training, as described in Section~\ref{sec:cpl}. Algorithm~\ref{alg:cpt} contains the final algorithm.  
\begin{algorithm}
  \caption{Conjugate pseudo-labeling}
  \label{alg:cpt}
  \label{alg:conjPL}
  \begin{center}
    \hspace*{\algorithmicindent}
    \textbf{Input:} Source classifier $\sourcetheta$ obtained by running gradient descent on $\lsource(\theta) = \sum\limits_{(x, y) \in \dsource} \ell( h_\theta(x), y)$, where $\ell(z, y) = f(z) - y^\top z$.\\ 
     \hspace*{\algorithmicindent}
     \textbf{Hyperparameters:} learning rate $\eta$ and temperature scaling $T$
     \end{center}
  \begin{algorithmic}[1]
    \STATEx 
    Let $\scaledpred_\theta(x) \eqdef h_\theta(x)/T$ be the temperature scaled predictor. 
    \STATEx
    \vspace{2pt}
    Let $\cpl_\theta(x)$ denote the conjugate pseudo-label function $\cpl_\theta(x) =\nabla(f(\bar{h}_\theta(x)))$.
    \STATEx
    \vspace{2pt}
    \textbf{for} $n = 0, 1, \hdots N-1$ \textbf{do}
    \STATEx
    \hspace{10pt} Sample $x_n \sim \dtest$.
    \STATEx
    \hspace{10pt}
    \STATEx
    \hspace{10pt} $\theta_{n+1} = \theta_n - \eta \nabla \ell\Big(\scaledpred_\theta(x_n), \cpl_\theta(x_n)\Big)$ ~~\text{[Self-training with conjugate pseudo-labels]}
  \end{algorithmic}
\end{algorithm}

For brevity in presentation, we only considered losses of the form $\ell(z, y) = f(z) - z^\top y$. We show how to extend this approach to slightly more general losses and also compute the expression of the conjugate pseudo-labels for a few different loss functions in Appendix [TODO].

% \subsection{Conjugate Adaptation Loss}
% Consider a source classifier $h_{\theta}$, trained using loss functions of the form : 
% \begin{align}
% \label{eq:loss_general}
%     \textstyle 
%     \begin{split}
%     \mathcal{L}(z,y) &= f(z) - y^{T}z\\
%     \end{split}
% \end{align}
% where $z = h_{\theta}(x)$ and $(x,y)\sim D_s$ from some source distribution $D_s$. A large class of commonly used loss functions can be written in above form as we describe later. The convex conjugate of any function $f : Z^{C} \rightarrow \mathbb{R}$ is defined as follows : 
%  \begin{align}
%  \label{eq:conjugate_definition}
%      \textstyle 
%      f^{*}(y) &= -\min_{z}[f(z) - y^{T}z]
%  \end{align}
% % Now, let us consider the cross entropy loss which can be written in the form of \autoref{eq:loss_general} as:
% % \begin{align}
% % \label{eq:Xent_loss}
% %     \textstyle 
% %     \mathcal{L}_{\text{Xent}}(z,y) &= \log \sum_{k=1}^K e^{z_k} - y^{T}z
% % \end{align}
% % Taking the convex conjugate of $f(z)=\log \sum_{k=1}^K e^{z_k}$, we obtain :
% % \begin{align}
% % \label{eq:Xent_conjugate}
% %     \textstyle 
% %     \begin{split}
% %     f^{*}(y) &= -\min_{z} (\log \sum_{i}e^{z_{i}} - y^{T}z)\\
% %     f^{*}(y) &= \sum_{i}y_{i}\log y_{i} \text{ \;\; where \;\;} y_{i} = {e^{z_{i}}\over \sum_{i}e^{z_{i}}}
% %     \end{split}
% % \end{align}

% % Observe that the convex conjugate obtained above is the negative of softmax-entropy; which the meta-loss learnt as TTA objective for a cross entropy trained classifier in the experiments in \autoref{sec:meta-loss}.\\
% % Similarly, consider the squared loss which can be written as :
% % \begin{align}
% % \label{eq:squared_loss}
% %     \textstyle 
% %     \mathcal{L}_{\text{sq}}(z,y) &= \frac{1}{2}z^{2} - y^{T}z
% % \end{align}
% % with the conjugate defined as $f^{*}(y) = y^{2}\text{ where } y=z$ at the optimal. Again, this is the TTA objective which the meta-loss learnt in the experiments in \autoref{sec:meta-loss} for a source classifier trained using squared loss.\\
% \textbf{Proposed Conjugate Loss for Adaptation} Given a classifier $h_{\theta}$ trained using a loss function of the form specified by \autoref{eq:loss_general}, we propose to use the negative of the conjugate of $f$ as the TTA objective for unsupervised domain adaptation. We re-parameterize the conjugate in the $z$ space, based on the optimal relation between $y$ and $z$ at the minima in \autoref{eq:conjugate_definition}.
% \begin{align}
% \label{eq:conjugate_loss}
%     \textstyle 
%     \mathcal{L}_{\text{conjugate}}(z) &= -f^{*}(y_\text{opt}(z)) = f(z) - \frac{\partial f(z)}{\partial z}^{T}z
% \end{align}
% %where $y_\text{opt}$ is a function of $z$ that is given by taking the derivation of training loss to zero:
% %\begin{align}
% %\label{eq:y_opt}
% %\textstyle 
% %y_\text{opt}&=\frac{\partial f(z)}{\partial z}
% %\end{align}

% For example, consider the cross-entropy loss, which can be expressed in the form of \autoref{eq:loss_general} as $\mathcal{L}_\text{Xent}(z, y) = \log \sum_{k=1}^K e^{z_k}-y^{T}z$, with $f(z)$ being the $\mathrm{LogSumExp}(z)$ function. Here, the conjugate adaptation loss as proposed above will be given by:
% \begin{align}
% \label{eq:conjugate_xent}
%     \textstyle 
%     \mathcal{L}_{\text{conjugate}}^{\text{Xent}}(z)&=-f^{*}(y_{\text{opt}})(z) = \sum_{i}y_{i}\log y_{i} \text{ \;\; where \;\;} y_{i} = {e^{z_{i}}\over \sum_{i}e^{z_{i}}}
% \end{align}
% Note that the conjugate above exactly recovers the meta-loss learnt in \autoref{sec:meta-loss} for $h_{\theta}$ trained using cross-entropy loss(upto a constant temperature scaling factor over the logits). \sg{Further, the temperature scaling is simply a perspective transform over the f(z). We can talk about this more, but I fear reader getting confused then}.

% Similarly consider the squared loss for training the source model $h_{\theta}$, which can be expressed as $\mathcal{L}_{\text{sq}}(z,y) = \frac{1}{2}z^{2} - y^{T}z$ where $z=h_{\theta}(x)$. From \autoref{eq:conjugate_loss}, we have $\mathcal{L}_{\text{conjugate}}^{\text{sq}}(z)=-\frac{1}{2}z^2$, which again recovers the meta-loss learnt in \autoref{sec:meta-loss} for $h_{\theta}$ trained using squared loss.

% %\textbf{Softmax cross-entropy} is the de facto loss function for multi-class classification in modern deep learning, and can be expressed in the form given by Equation \ref{eq:loss_general} as :
% %\begin{align}
% %\textstyle
% %\mathcal{L}_\text{softmax}(\bm{z}, \bm{y}) &= 
% % -\sum_{k=1}^K y_k \log\left(\frac{e^{z_k}}{\sum_{j=1}^K e^{z_j}}\right) 
% %\log \sum_{k=1}^K e^{z_k}-y^{T}z
% %\end{align}
% %with $f(z)$ being the $\mathrm{LogSumExp}(z)$ function and $g(z)=z$. Here, $\mathcal{L}_\text{uda}$ given by Equation \ref{eq:loss_uda} exactly recovers the softmax entropy (details in Apppendix \ref{uda_derivations}), which matches our observations from \autoref{sec:meta-loss} that meta loss learns a scaled softmax entropy function for CE-trained networks.

% \subsection{Extension to other training losses}

% %Given a test input $(x,y)\sim D_t$ where $D_t$ denotes the target domain, we propose to use the negative conjugate of $f\circ g^{-1}$ as the test time adaptation loss, i.e.
% %\begin{align}
% %\label{eq:loss_uda}
% %    \textstyle 
% %    \begin{split}
% %    \mathcal{L}_{uda}(k) &= -p^{*}(y^{*}(k)) = -[y^{*}(k)^Tk - f(g^{-1}(k)]\\
% %    \mathcal{L}_{uda}(z) &= -\left[\frac{\partial_{z} f(z)}{\partial_{z} g(z)}g(z) - f(z)\right]\\
% %    \mathcal{L}_{uda}(z) &= f(z) - \frac{\partial_{z} f(z)}{\partial_{z} g(z)}g(z)
% %    \end{split}
% %\end{align}


% Our conjugate loss formulation can be easily extended further to loss function of the form:
% \begin{align}\label{eq:loss_g}
% \textstyle 
%     \begin{split}
%     \mathcal{L}(z, y)&=f(z)-y^{T}g(z)\\
%     \mathcal{L}(z, y)&=f\circ g^{-1}(z')-y^{T}z' \text{ \;where\; } z'=g(z)
%     \end{split}
% \end{align}
% which brings us back to the functional form in \autoref{eq:loss_general}. The conjugate adaptation loss for $h_{\theta}$ trained using this loss function would be given by the convex conjugate of $f\circ g^{-1}$: 
% \begin{align}
%     \textstyle 
%     \mathcal{L}_{\text{conjugate}}(z) &= -(f\circ g^{-1})^{*}(y_\text{opt}(z)) = f\circ g^{-1}(z') - \frac{\partial (f\circ g^{-1}(z'))}{\partial z'}z'\\
%     %&\mathcal{L}_{\text{conjugate}}(z) = f\circ g^{-1}(z') - \frac{\partial_z f\circ g^{-1}(z')}{\partial_z g[g^{-1}(z')]}z'\\
%     &\mathcal{L}_{\text{conjugate}}(z) = f(z) - \frac{\partial_z f(z)}{\partial_z g(z)}^{T}g(z)\label{eq:conjugate_loss_fg}
% \end{align}

% % Assume $f$ and $g$ are differentiable, at the optimal solution, the derivative is equal to 0, which gives:
% %\begin{align}\label{optimal-relation}
% %\textstyle 
% %    y_\text{opt} &= \frac{\partial_{z} f(z)}{\partial_{z} g(z)}
% %\end{align}
% %In this case, the correct pseudo label for test-time adaptation should be derived the optimal relation in~\autoref{optimal-relation}. At test time, our proposed unsupervised loss function is:
% %\begin{align}
% %    \textstyle 
% %    \mathcal{L}_\text{uda}(\bm{z}) &=f(z)-\frac{\partial_{z} f(z)}{\partial_{z} g(z)}^{T}g(z)
% %\end{align}

% % Now we apply our framework to common losses used in machine learning and derive the corresponding loss function for test-time adaptation. 


% \textbf{Margin-based losses} 
% For binary classification tasks where the model outputs $z=h_{\theta}(x)$ and the label space is $y\in\{-1,1\}$, 
% margin-based loss function of the form  $\mathcal{L}_\text{margin}=l(-y\cdot z)$ is widely used. Special cases where $l(t)=\log(1+e^{t})$ and $l(t)=e^{t}$ correspond to logistic loss and exponential loss respectively. It is easy to check that the loss can be rewritten as:
% \begin{align}
% \textstyle
%     \mathcal{L}_\text{binary}(\bm{z},\bm{y}) &=\frac{1}{2}\bigg(l(-z)+l(z)\bigg)-y\cdot \frac{1}{2}\bigg(l(z)-l(-z)\bigg)
% \end{align}
% For such loss functions, the conjugate adaptation loss can be derived using \autoref{eq:conjugate_loss_fg} : 
% \begin{align}
% \label{eq:margin_loss_conjugate}
% \textstyle
%     \mathcal{L}_\text{conjugate}^{\text{binary}}(z) &=\frac{1}{2}\bigg(l(-z)+l(z)\bigg)-y_{\text{opt}}(z)\cdot \frac{1}{2}\bigg(l(z)-l(-z)\bigg)\\
%     &\text{ where\; }y_{\text{opt}}(z)=\frac{l'(z)-l'(-z)}{l'(z)+l'(-z)}
% \end{align}
%  %For such loss function, by taking the gradient to be zero, the pseudo label given by our framework is:
% %\begin{align}\label{margin-soft-pl}
% %\textstyle 
% %    y&=\frac{l'(z)-l'(-z)}{l'(z)+l'(-z)}
% %\end{align}
% %Applied to the logistic loss function, the soft pseudo label given by the optimal relation is $y_\text{soft pl}=(e^{z}-1)/(e^{z}+1)$. The corresponding conjugate loss for adaptation is entropy with sigmoid probability $-\sigma(z)\log\sigma(z)-(1-\sigma (z))\log(1-\sigma (z))$ whre $\sigma$ is the sigmoid function.

% \textbf{PolyLoss}~\citet{polyloss} is a recently proposed loss function showing promising improvements compared to standard training losses over classification tasks. PolyLoss generalizes cross entropy and focal loss and is a novel framework of loss functions from a polynomial expansion perspective. The simplest Poly-1 for the PolyLoss family is proposed by tuning the first polynomial term. Poly-1 is defined as:
% \begin{align}
% \label{eq:poly_loss}
%     \mathcal{L}_\text{Poly-1}(\bm{z},\bm{y}) &= \log \sum_{i=1}^C e^{z_i}-y^{T}\left(z-\epsilon+\epsilon\cdot p_z\right)
% \end{align}
% where $C$ is the number of classes, $p_z$ is the softmax normalized prediction vector i.e. $p_z = \mathrm{softmax}(h_{\theta}(x))$. For PolyLoss, the conjugate adaptation loss given by \autoref{eq:conjugate_loss_fg} will be : 
% \begin{align}
% \label{eq:poly_loss_conjugate}
%     &\mathcal{L}_\text{conjugate}^\text{Poly-1}(\bm{z},\bm{y}) = \log \sum_{i=1}^C e^{z_i}-y_{\text{opt}}(z)^{T}\left(z-\epsilon+\epsilon\cdot p_z\right)\\
%     &\text{ where\; }y_{\text{opt}}(z)=\left(I+\epsilon\times \mathtt{diag}(p_z)-\epsilon*p_{z}p_{z}^{T}\right)^{-1}p(z)
% \end{align}

% \subsection{Connection to instantaneous pseudo-labelling}
% Consider the conjugate loss for polyloss and the margin loss specified in \autoref{eq:poly_loss_conjugate} and \autoref{eq:margin_loss_conjugate}. The conjugate draws an interesting connection with self-training with instantaneous pseudo-labels given by $y_\text{opt}(z)$

==> old_metaloss.tex <==
\section{Test-time Adaptation via Meta-Learnt Losses}\label{sec:meta-loss}
We start by revisiting the choice of loss function for test-time adaptation. TENT~\citep{tent} chooses entropy as they observe empirically that entropy is highly correlated to error and degree of shift on corruption data. However, there is no fundamental explanation as for why it works well in practice. Entropy minimization tries to assign a higher probability to the predicted class, and the same can be achieved by various other loss formulations. For example, a recent work RPL \citet{rpl}, proposes minimizing ${L}_{rpl}=q^{-1}(1-p_z^q)$ where $p_z$ is the probability of the predicted class, and shows its effectiveness empirically. However, there is no fundamental reasoning behind either of them being a good choice for test time adaptation loss. Similar arguments can be made for other self-learning based losses, e.g. pseudo labelling~\citep{rusak2022if}. 

\begin{figure}[!htbp]
	\centering
	\begin{subfigure}{0.45\textwidth}
		\includegraphics[width=\textwidth]{figures/meta_loss_ce.jpg}
		\caption{}
		\label{meta-loss-ce-trained}
	\end{subfigure}
%%%%%%%%%%%%%%
	\begin{subfigure}{0.45\textwidth}
		\includegraphics[width=\textwidth]{figures/meta_loss_quad.jpg}
		\caption{}
		\label{meta-loss-quadratic}
	\end{subfigure}
  \caption{Visualization of meta loss (blue) and softmax entropy (red) functions in one dimension. . For CE-trained model in~\autoref{meta-loss-ce-trained}, the meta loss can be fitted in shape with a scaled version of softmax entropy.}
\label{fig:fitted_ce}
\end{figure}

The natural question which arises here is how do we go about exploring other loss functions ? We take a meta-loss learning approach as described in \autoref{sec:preliminary} and consider learning a meta-loss in the set of loss functions over the model outputs $h_{\theta}(x)$ i.e. $\{l(h_{\theta}(x)) : \mathbb{R}^C \rightarrow \mathbb{R}\}$, where $C$ is the number of categories in the classification task.


The above discussion motivates us to explore new unsupervised loss functions for test-time adaptation. We use a meta learning approach. Specifically, we parametrize the loss function as a neural network over logits, which we termed as meta loss. Then meta learning is applied to learn a meta loss for the task of test time adaptation. (\ms{cite the meta learning loss function part here}) We take a ResNet-26 trained on CIFAR-10, which is the standard network for evaluating test-time adaptation on CIFAR-10. Then meta learns a loss function from a CIFAR-10-C validation noise dataset. The learnted meta loss is tested on all 15 noises in CIFAR-10-C test set with the highest severity level and compared with softmax entropy baseline.

As expected, the meta loss has a mean error of 12.20$\%$ better than the softmax entropy baseline 13.11$\%$. We then analyze what is learnt by the meta loss. We view the meta loss as a standalone neural network and plot the meta loss function by varying one input dimension, in other words, the prediction score of one class. The result is shown in~\autoref{meta-loss-ce-trained} (blue curve). With more careful observation, we find that the meta loss function can be closely approximated by a scaled version of softmax entropy (dashed red curve):
\begin{align}
    \mathcal{L}_\text{scaled}=\alpha\cdot \mathcal{H}(\text{softmax}(x/T))
\end{align}
 where we introduce a magnitude parameter $\alpha$ and temperature $T$. Further, the fitted entropy function has a mean error of 12.14$\%$ which matches the performance of meta loss for test-time adaptation on CIFAR-10-C. It turns out that we started off trying to find a better function than entropy via meta loss but still ended up re-discovering the entropy function yet with temperature scaling. 

The result suggests that there is something fundamental going on. Entropy itself is indeed a good choice of loss function for test-time adaptation. Meta loss is simply trying learn a scaled entropy function but with no explicit supervision of entropy signal during meta training. Now we take a step back and \ms{not sure how the transition should be here}.

We experimented with a ResNet trained with Quadratic loss function. We are able to learn a meta loss (13.48$\%$ mean error) for this network that outperforms softmax entropy (14.57$\%$). Similarly, we plot the meta loss function by varying one logit input, shown in ~\autoref{meta-loss-quadratic}. In this case, the meta loss is closer in shape to a quadratic function. Thus we fit a quadratic function $g$ to the meta loss and the new quadratic loss achieves (13.20$\%$) as compared to the meta loss (13.48$\%$). The analysis on quadratic-trained classifier shows that there exists a better function than softmax entropy for test-time adaptation and the training loss does affect the loss function to be used.

% Without a principled understanding, 
% it prompts us think about better unsupervised objectives beyond softmax entropy.



% While TENT is shown to work well across architectures and tasks, there is no principled understanding of why entropy minimization on test data works for test-time adaptation.

\ar{Overall, this section can be made more "dramatic", in a storytelling fashion rather than just stating what you observed...build the suspense and really emphasize what is surprising and why}
We start by asking a simple question: is there a better unsupervised objective for test-time adaptation than entropy? \ar{Should motivate this better? Why did people try entropy/what's the intuition and why some other losses might also make sense? What's an example of another loss that might make sense? Also, maybe you could motivate whether the adaptation objective depends on the base classifier in some way? No work has previously explored this so it is nice to point out} We tackle this problem by learning this unsupervised loss function directly.
\ar{The next part should go into preliminaries/setup. Only the actual meta loss setup should be here} 
Consider learning a loss function $l:\mathbb{R}^{K}\rightarrow \mathbb{R}$ from the family of value functions over logit vector $z\in\mathbb{R}^{K}$, this value function would be softmax entropy for TENT~\citep{tent}:
\begin{align}
    l_\text{tent}(z)&=H(\text{softmax}(z))
\end{align}


% The meta loss is updated iteratively until convergence. We start with a standard ResNet-26 on CIFAR-10 and apply our meta learning procedure to train a meta loss. We use labelled data from CIFAR-10-C validation set (consists of four noises). The learnt meta loss is then tested on 15 noises in CIFAR-10-C test set. We made several observations on the meta loss:
% \begin{itemize}[leftmargin=1.5em,itemsep=0em,topsep=0em]
%     \item Meta loss (12.20$\%$ mean error) outperforms softmax entropy ($13.11\%$ mean error) by a reasonable margin under default optimization setting (SGD with learning rate $0.001$).
%     \item When visualizing the meta loss function in one input dimension, it learns a scaled version of softmax entropy. Specifically, by adding a temperature $T$ and scaling parameter $\alpha$ to the softmax entropy function:$l_\text{fitted}=\alpha\cdot H(\text{softmax}(x/T))$, 
%     one can approximate the overall shape of meta loss, as shown in \autoref{meta-loss-ce-trained}.
%     \item Furthermore, this fitted entropy function (12.14$\%$) performs similar result to meta loss (12.20$\%$), suggesting that softmax entropy itself is a good function for test-time adaptation with properly tuned temperature and scaling factor. (In reality, this scaling factor can be represented by learning rate.)
% \end{itemize}

% This raises the question whether meta loss is always learning softmax entropy? We experimented with a ResNet trained with Quadratic loss function. We are able to learn a meta loss (13.48$\%$ mean error) for this network that outperforms softmax entropy (14.57$\%$). Similarly, we plot the meta loss function by varying one logit input, shown in ~\autoref{meta-loss-quadratic}. In this case, the meta loss is closer in shape to a quadratic function. Thus we fit a quadratic function $g$ to the meta loss and the new quadratic loss achieves (13.20$\%$) as compared to the meta loss (13.48$\%$). The analysis on quadratic-trained classifier shows that there exists a better function than softmax entropy for test-time adaptation and the training loss does affect the loss function to be used.

  The above experiments suggest that the \textit{choice of test time adaptation objective should take into consideration the supervised learning objective used for training the source model}. In the next section, we formalize this relation by explicitly modelling the training loss function and propose a new unsupervised objective for test-time adaptation.
  \ar{The experiments also motivate the conjugate story...i think that should also go in this section, otherwise the connection between 3 and 4 is very loose. Why did you arrive at that formulation?}




% In this section, we first ask the question whether entropy is always a good choice for test time adaptation. 
% Specifically, we consider 2 different source classifiers trained with different supervised learning objective on the source domain data. We assume access to some labelled data from target domain (only for analysis in this section). We want to learn a test time adaptation objective, which we can use to fine-tune the source classifier such that it is able to classify the target domain samples correctly.

%Concurrently, \citet{gradualUDA} show the use of self-training with pseudo-labels for the task of UDA. 
%We first ask the question whether entropy is the optimal objective for unsupervised test time updates on the source model? If we were given access to the labelled data from target domain, could we have learnt a better objective for test time adaptation?
% \textbf{Setup}: Consider a classifier $f_{\theta}$ trained using some supervised learning objective on the labelled data from the source domain. Consider two type of classifiers : (1) $f_{\theta}^{Xent}$, trained using cross entropy loss and (2) $f_{\theta}^{quad}$, trained using quadratic loss. Further, for the purpose of analysis in this section, consider access to labelled data from target domain i.e. $(x_t, y_t)\sim D_t$. Our goal is to learn an unsupervised loss function $\mathcal{L}_{\phi} \in \mathbb{R}^{c} \rightarrow \mathbb{R}$, which takes as input the predictions ($\in \mathbb{R}^{c}$) given by the source classifier for a test input and returns a scalar loss value.

%\textbf{Setup}: Consider a source classifier $f_{\theta}$ trained on labelled data from the source domain. We consider two type of source classifiers : (1) $f_{\theta}^{Xent}$, trained using cross entropy loss and (2) $f_{\theta}^{quad}$, trained using quadratic loss. Further, for the purpose of analysis in this section, consider access to labelled data from target domain i.e. $(x_t, y_t)\sim D_t$. Our goal is to learn an unsupervised loss function $\mathcal{L}_{\phi}$ (parametrized by $\phi$), which takes in the predictions from the source model and gives a loss value.

% \textbf{Meta Learning the Objective}: Given a test batch, we fine tune the source model with the loss given by $L_{\phi}$ for the predictions of source model i.e. $\theta_{x_t} \leftarrow \theta - \frac{\partial \mathcal{L}_{\phi}(f_{\theta}(x_t))}{\partial \theta}$. The loss function parameters $\phi$ can than in turn be updated as $ \phi \leftarrow \phi - \frac{\partial loss(f_{\theta_{x_t}}(x_t),  y_{x_t})}{\partial \phi} $, using the derivative  with respect to $\phi$ of a loss function which evaluates updated source model parameters $\theta_{x_t}$ on the target labelled data. Note that higher order derivatives would be involved here. We do this iteratively until convergence.

% \textbf{Visualizing the learnt objective} :  Consider the two source models trained on CIFAR-10 dataset, one using cross entropy loss ($f_{\theta}^{Xent}$) and another using a quadratic loss ($f_{\theta}^{quad}$). Consider the task of domain adaptation from CIFAR-10 to CIFAR-10-Corruptions dataset (cite). We learn a test time adaptation objective for this task as described above, assuming access to the labelled noise samples from the target domain (just for the analysis in this section). 


%Consider a source classifier trained using cross entropy loss ($f_{\theta}^{Xent}$) on the CIFAR-10 dataset. We learn a loss function $\mathcal{L}_{\phi}$ as described above for the domain adaptation task from CIFAR-10 to CIFAR-10 corruptions dataset. $\mathcal{L}_{\phi}$ takes as input the 10D logits given by the source model and returns a loss value. Figure \ref{fig:fitted_ce} (blue curve) shows the loss output as we vary a logit from -10 to 10, keeping the others fixed at 0. The learnt loss can be approximated well with a scaled softmax entropy function, shown in Figure \ref{fig:fitted_ce} red curve. As discussed in Section \ref{section:exp}, the scaled softmax entropy easily beats the baselines on the domain adaptation tasks. 






==> tables/table-digit-data.tex <==
\begin{table}[!ht]
    \centering
    % \setlength{\tabcolsep}{1.4pt}
    \resizebox{1.0\textwidth}{!}{
\begin{tabular}{cccccc||c}
    \toprule
    Dataset  &  \begin{tabular}[c]{@{}c@{}}Source\\ Error\end{tabular} & 
    \begin{tabular}[c]{@{}c@{}}Hard\\ PL\end{tabular}  & \begin{tabular}[c]{@{}c@{}}Robust\\ PL \end{tabular} & \multicolumn{1}{c}{Entropy}  &
    \begin{tabular}[c||]{@{}c@{}}Softmax\\ PL\end{tabular} &
    \begin{tabular}[c]{@{}c@{}}Conjugate PL\\ \textbf{Ours}\end{tabular} \\
    \midrule
    \multirow{1}{*}{SVHN $\rightarrow$ MNIST} & 28.33 & 20.21  & 19.73  & 14.28 & 16.54 & \textbf{10.73} \\\midrule 
    \multirow{1}{*}{SVHN $\rightarrow$ USPS} & 31.58  & 23.32  & 26.12 & 23.12 & 24.07 & \textbf{21.62} \\\midrule 
    \multirow{1}{*}{SVHN $\rightarrow$ MNISTM} & 61.69  & 50.73  & 51.35 & 49.33 & 50.47 & \textbf{47.59} \\
    \bottomrule
    \end{tabular}
    }
    \vspace{1ex}
    \caption{Error on various digit adaptation benchmarks, for a source classifier trained using polyloss.}
    \label{tab-appendix:digit-adapt}
\end{table}
\vspace{-2em}


